An examination of the effect on the Icelandic Banking System of Ver{\dh}trygg{\dh} L\'{a}n (Indexed-Linked Loans)

In 1979 following a decade of hyperinflation, Iceland introduced Ver{\dh}trygg{\dh} l\'an, negatively amortised, index-linked loans whose outstanding principal is increased by the rate of the consumer price inflation index(CPI). The loans were part of a general government policy which used indexation to the CPI to address the economic consequences of the hyperinflation. Although most other forms of indexation were subsequently removed, loan indexation has remained, and these loans now comprise the majority of mortgages in Iceland. Although it is still often argued that index-linked loans helped to stop the hyperinflation, these arguments are typically based on high level macro-economic interpretations of the Icelandic economy, they fail to identify specific mechanisms to support their claims. In this paper we take the opposite approach, and present a detailed analysis of the monetary mechanics used for the loans at the double entry bookkeeping level of the banking system. Based on this analysis there appears to be no evidence or mechanism that would support the claim that index-linked loans reduce or stop inflation. On the contrary: our research shows that the bookkeeping treatment of these loans within the banking system directly contributes to the banking system's monetary expansion rate, and hence index-linked loans act to increase the inflation rate to which they are linked, rather than reducing it. They consequently create a positive feedback loop within the banking system's monetary regulation operating directly on the money supply. Since the feedback into monetary expansion only occurs at annual CPI rates above approximately 2%, we suggest one solution would be to stabilise the money supply to 0% growth, and we explore some ways this could be achieved by modifying the Basel Regulatory Framework within the Icelandic Banking System.

==> titlepage_iiim.tex <==
\renewcommand{\rmdefault}{eurostile}		% Set font to Eurostile for Kris
\begin{titlepage}
\begin{textblock}{2}(0,0)
  {\includegraphics{IIIM-header-stripes-vertical.eps}}
\end{textblock}
\begin{textblock}{5}(11,1)
  {\includegraphics[width=5cm]{IIIM-logo.eps}}
\end{textblock}
\begin{textblock}{8}(7,14.6) {IIIM TECH REPORT IIIMTR-2013-01-001}
\end{textblock}
\begin{textblock}{5}(12.4,14.5)
  {\includegraphics[width=3cm]{wwwiiimis-black-box.eps}}
\end{textblock}
\begin{textblock}{5}(7,15.1)
   \includegraphics[width=10.1cm]{IIIM-black-box.eps}
\end{textblock}

\begin{textblock}{10}(3,5)
{
\textbf{\huge
An Examination of the effect on the 
\vspace{5mm}    \\              %  Must use vspace, and newline to separate
Icelandic Banking System of 
\vspace{5mm}    \\              %  Must use vspace, and newline to separate
Ver{\dh}trygg{\dh} L\'{a}n (Indexed-Linked Loans).
}}
{ \large
\vspace{2cm} \\
\textbf{Jacky Mallett}
\vspace{4mm}    \\              %  Must use vspace, and newline to separate
\textbf{jacky@ru.is}
\vspace{4mm} \\
\textbf{Research Scientist}
\vspace{4mm} \\
\textbf{IIIM}
}
\end{textblock}
\end{titlepage}
\null\newpage

